On multi-time-step monolithic coupling algorithms for elastodynamics

We present a way of constructing multi-time-step monolithic coupling methods for elastodynamics. The governing equations for constrained multiple subdomains are written in dual Schur form and enforce the continuity of velocities at system time levels. The resulting equations will be in the form of differential-algebraic equations. To crystallize the ideas we shall employ Newmark family of time-stepping schemes. The proposed method can handle multiple subdomains, and allows different time-steps as well as different time stepping schemes from the Newmark family in different subdomains. We shall use the energy method to assess the numerical stability, and quantify the influence of perturbations under the proposed coupling method. We also discuss the conditions under which the proposed method will be energy preserving, and the conditions under which the method will be energy conserving. Several numerical examples are presented to illustrate the accuracy and stability properties of the proposed method. We shall also compare the proposed multi-time-step coupling method with some other similar methods available in the literature.

==> Sections/Notation.tex <==
\section*{NOMENCLATURE}
\label{notation}

\begin{tiny}   
\begin{longtable}{|c|l|c|l|} \hline 
\textsf{Symbol} & \textsf{Quantity} & \textsf{Symbol} & \textsf{Quantity} \\ \hline
$ \llangle \cdot \rrangle$ & Average operator over system time-step & 
$\boldsymbol{d}_{\mathrm{drift}}^{(n)}$ 
& Drift in displacement at $n$-th system time-level \\
%
$\llbracket \cdot \rrbracket$ & Jump operator over system time-step 
& $\boldsymbol{f}$ &  Vector of external force \\
%
$ [ \cdot ]_i$ & Jump operator over the $i$-th subdomain time-step & 
$\boldsymbol{f}_i$ & Vector of external forces on $i$-th subdomain \\
%
$\langle \cdot \rangle_i$ & Average operator over the 
$i$-th subdomain time-step & $\boldsymbol{K}$ & 
Stiffness matrix of the undecomposed domain \\
%
$\beta$ & Newmark parameter & $\boldsymbol{K}_i$ & Stiffness matrix of $i$-th subdomain \\
%
$\beta_i$ & Newmark parameter for $i$-th subdomain & $\boldsymbol{M}$ & Mass matrix of the undecomposed domain \\
%
$\Delta t$ & System time-step & $\boldsymbol{M}_i$ & Mass matrix of the $i$-th subdomain \\ 
%
$\Delta t_i$ & Subdomain time-step & $N$ & Number of system time-levels \\
%
$\eta_i$ & Number of subdomain time-levels in a system time-step 
& $S$ & Number of subdomains \\
%
$\gamma$ & Newmark parameter $\gamma \geq 1/2$ & $t$ & time \\ 
%
$\gamma_i$ & Newmark parameter for $i$-th subdomain $\gamma_i \geq 1/2$ 
& $T$ & total time of interest \\
%
$\boldsymbol{\lambda}$ & Lagrange multiplier to enforce 
constraints & $\boldsymbol{u}$ & displacement vector \\
%
$\boldsymbol{a}_{\mathrm{drift}}^{(n)}$ 
& Drift in acceleration at $n$-th system time-level & 
$\dot{\boldsymbol{u}}$ & Velocity vector \\
%
$\boldsymbol{C}_i$ & Signed Boolean matrix for $i$-th subdomain & $\ddot{\boldsymbol{u}}$ & Acceleration vector \\ \hline
%
\end{longtable}
\end{tiny}
